Identifying and Correcting Label Bias in Machine Learning

Datasets often contain biases which unfairly disadvantage certain groups, and classifiers trained on such datasets can inherit these biases. In this paper, we provide a mathematical formulation of how this bias can arise. We do so by assuming the existence of underlying, unknown, and unbiased labels which are overwritten by an agent who intends to provide accurate labels but may have biases against certain groups. Despite the fact that we only observe the biased labels, we are able to show that the bias may nevertheless be corrected by re-weighting the data points without changing the labels. We show, with theoretical guarantees, that training on the re-weighted dataset corresponds to training on the unobserved but unbiased labels, thus leading to an unbiased machine learning classifier. Our procedure is fast and robust and can be used with virtually any learning algorithm. We evaluate on a number of standard machine learning fairness datasets and a variety of fairness notions, finding that our method outperforms standard approaches in achieving fair classification.

==> AdditionalFairness.tex <==

\section{Fairness Experiments with Additional Baselines}

\subsection{Additional Baselines}

We now compare against additional Lagrangian baselines recommended by \cite{cotter2018optimization}, which gave a thorough analysis of Lagrangian-based methods and their application to fair machine learning:
\begin{itemize}
    \item {\bf Hinge Lagr.} This was the Lagrangian baseline of \cite{eban2017scalable} used in Table~\ref{tab:experiments} which proceeds by performing a Hinge relaxation of the fairness constraints to make the Lagrangian differentiable so that it can be trained by gradient-based methods.
    \item {\bf 0/1 Lagr.} This was the method recommended by \cite{cotter2018optimization} which they call "0/1 Best External." It proceeds by playing a two-player game where one player minimizes the Hinge-relaxed Lagrangian but the other player enforces fairness by learning the Lagrange multipliers based on the original fairness constraint (rather than a Hinge relaxation). This leads to a non-zero-sum two-player game and each player proceeds by alternating performing SGD on their respective objectives. Then at the end, a heuristic is used to choose the "best" iterate based on the fairness and accuracy on the training set.
    We tune the hyperparameters (i.e. fairness slack and number of iterations) the same as in the Hinge Lagr. baseline.
    \item  {\bf 0/1 Lagr. Full} This is the same as the previous, but instead of each player taking a stochastic gradient descent step, each player takes a full gradient step computed over the entire training set.
\end{itemize}
We note that \cite{cotter2018optimization} also recommend another baseline which learns a randomized classifier, but the scope of our work deals with deterministic classifiers.

\subsection{Results}
We show results by fairness metric: Demographic Parity (Table~\ref{tab:experiments_demparity}), Disparate Impact (Table~\ref{tab:experiments_disparate}), Equal Opportunity (Table~\ref{tab:experiments_equalopp}), and Equalized Odds (Table~\ref{tab:experiments_equalodds}).

We see that our method outperforms the state of art for Demographic Parity and performs competitively with the Lagrangian methods on the other notions of fairness despite being a simpler approach.


\begin{table*}
\setlength{\tabcolsep}{5pt}
\begin{center}
  \caption{{\bf Additional Demographic Parity Results}}
  \label{tab:experiments_demparity}
  \begin{tabular}{|l|r|r|r|r|r|r|}
 \hline
Dataset & Unconstrained & Calibration &  Hinge Lagr. & 0/1 Lagr. &  0/1 Lagr. Full & Our Method \\
\hline
Bank Err. & 9.41\% & 9.7\% &	10.46\% &	9.65\% &	11.22\% &	9.63\% \\
Bank Vio.  & 0.0349	 & 0.0068 &	0.0126 &	0.018	& 0.0068 & {\bf  0.0056} \\
\hline
COMPAS Err. & 31.49\% & 	32.53\% & 	40.16\% & 	38.02\% & 	39.69\% & 	35.44\%  \\
COMPAS Vio.&  0.2045 &	0.0201&	0.0495 &	0.0462 &	0.0477 &	{\bf 0.0155} \\
\hline
Communities Err.&  11.62\% & 	32.06\% & 	28.46\% & 	24.45\% & 	23.84\% & 	30.06\% \\
Communities Vio. & 0.4211 &	0.0653	& 0.0519	& 0.1204 &	0.1538 &	{\bf 0.0107} \\
\hline
German Stat. Err.  & 24.85\% & 	24.85\% & 	25.45\% & 	27.27\% & 	27.88\% & 	25.15\%  \\
German Stat. Vio. & 0.0766 &	0.0346 &	0.041 &	0.0681 &	0.0802 &	{\bf 0.0137} \\
\hline
Adult Err.   & 14.15\% & 	16.6\% & 	20.47\% & 	19.57\% & 	19.71\% & 	16.51\%  \\
Adult Vio. & 0.1173	& 0.0129&	0.0198 &	0.0215 &	0.0277 &	{\bf 0.0037} \\
\hline
\end{tabular}
\end{center}
\end{table*}


\begin{table*}
\setlength{\tabcolsep}{5pt}
\begin{center}
  \caption{{\bf Additional Disparate Impact Results}}
  \label{tab:experiments_disparate}
  \begin{tabular}{|l|r|r|r|r|r|}
 \hline
Dataset & Unconstrained  &  Hinge Lagr. & 0/1 Lagr. &  0/1 Lagr. Full & Our Method \\
\hline
Bank Err. & 9.41\% &		10.44\% &	9.63\% &	9.94\% &	9.89\%  \\
Bank Vio.  & 0.0304	 &	0.0135 &	0.0179 &	0.0169 &	{\bf 0.0063} \\
\hline
COMPAS Err. & 31.21\% &		40.35\% &	38.97\% &	38.49\% &	42.64\% \\
COMPAS Vio.& 0.1362	 &	0.0499 &	0.0553	 & 0.0525 &	 {\bf 0.0256} \\
\hline
Communities Err.& 14.83\% &		28.26\% &	24.84\% &	25.05\% &	30.26\%  \\
Communities Vio. & 0.396	 &	0.0557 &	0.113 &	0.1224 &	{\bf 0.0073} \\
\hline
German Stat. Err.  & 24.85\% &		26.67\% &	25.45\% &	24.54\% &	25.15\%   \\
German Stat. Vio. & 0.0608 &	{\bf 0.0139} &	0.0167 &	0.0651 &	0.0156 \\
\hline
Adult Err.   & 14.19\% &		20.48\% &	19.76\% &	18.3\% &	17.37\%  \\
Adult Vio. &  0.1108 &	{\bf 0.0199} &	0.0233	& 0.0331	& 0.0334 \\
\hline
\end{tabular}
\end{center}
\end{table*}



\begin{table*}
\setlength{\tabcolsep}{5pt}
\begin{center}
  \caption{{\bf Additional Equal Opportunity Results}}
  \label{tab:experiments_equalopp}
  \begin{tabular}{|l|r|r|r|r|r|r|}
 \hline
Dataset & Unconstrained & Calibration &  Hinge Lagr. & 0/1 Lagr. &  0/1 Lagr. Full & Our Method \\
\hline
Bank Err. & 9.41\% &	9.55\% &	9.86\% &	9.64\% &	10.76\% &	9.48\% \\
Bank Vio.  & 0.1452 &	0.0506 &	0.1237 &	0.1061 &	0.1021 &	{\bf 0.0431} \\
\hline
COMPAS Err. & 31.49\% &	31.63\% &	36.92\% &	41.78\% &	38.59\% &	33.63\%  \\
COMPAS Vio.&  0.2373 &	{\bf 0.0256} &	0.1141 &	0.0411 &	0.092 &	0.0774 \\
\hline
Communities Err.&  11.62\% &	17.64\% &	28.45\% &	24.65\% &	26.65\% &	26.85\%  \\
Communities Vio. & 0.5513 & {\bf 	0.0584} &	0.0897 &	0.2115 &	0.1474 &	0.0833 \\
\hline
German Stat. Err.  & 24.85\% &	24.54\% &	27.27\% &	24.85\% &	24.54\% &	25.45\%  \\
German Stat. Vio. & 0.112 &	0.0922 &	0.0757 &	0.2032 &	0.096 &	{\bf 0.0662} \\
\hline
Adult Err.   & 14.15\% &	14.43\% &	19.67\% &	18.9\% &	17.95\% &	14.46\% \\
Adult Vio. & 0.1195 &	0.017 &	0.0374	& {\bf 0.0055} &	0.0099 &	0.0092\\
\hline
\end{tabular}
\end{center}
\end{table*}


\begin{table*}
\setlength{\tabcolsep}{5pt}
\begin{center}
  \caption{{\bf Additional Equalized Odds Results}}
  \label{tab:experiments_equalodds}
  \begin{tabular}{|l|r|r|r|r|r|}
 \hline
Dataset & Unconstrained  &  Hinge Lagr. & 0/1 Lagr. &  0/1 Lagr. Full & Our Method \\
\hline
Bank Err. &  9.41\% &		9.61\% &	9.66\% &	9.99\% &	9.5\%  \\
Bank Vio.  &  0.1452 &		0.0879 &	0.1093 &	0.1214 &	{\bf 0.0376} \\
\hline
COMPAS Err. & 31.49\% &		42.69\% &	42.35\% &	43.4\% &	35.06\%  \\
COMPAS Vio.& 0.2373	 &	0.0566 &	0.0576 &	{\bf 0.0477} &	0.0663 \\
\hline
Communities Err.& 11.62\% &		28.46\% &	23.84\% &	21.84\% &	26.65\%  \\
Communities Vio. & 0.5513 &		0.0962 &	0.2435 &	0.3205 &	{\bf 0.0769} \\
\hline
German Stat. Err.  & 24.85\%	&	27.57\% &	25.45\%	& 27.88\% 	& 25.45\%  \\
German Stat. Vio. & 0.112	 &	{\bf 0.0468} &	0.0919 &	0.074 &	0.1099 \\
\hline
Adult Err.   & 14.15\%	&	19.04\%  &	18.9\% &	18.13\% &	14.58\%   \\
Adult Vio. & 0.1195	&	0.016 &	{\bf 0.0156} &	0.0204 &	0.0221 \\
\hline
\end{tabular}
\end{center}
\end{table*}

